Privacy Preserving Group Membership Verification and Identification

When convoking privacy, group membership verification checks if a biometric trait corresponds to one member of a group without revealing the identity of that member. Similarly, group membership identification states which group the individual belongs to, without knowing his/her identity. A recent contribution provides privacy and security for group membership protocols through the joint use of two mechanisms: quantizing biometric templates into discrete embeddings and aggregating several templates into one group representation. This paper significantly improves that contribution because it jointly learns how to embed and aggregate instead of imposing fixed and hard coded rules. This is demonstrated by exposing the mathematical underpinnings of the learning stage before showing the improvements through an extensive series of experiments targeting face recognition. Overall, experiments show that learning yields an excellent trade-off between security /privacy and verification /identification performances.

==> ProblemFormulation.tex <==
% !TEX root = GroupMembershipVerification.tex

\vspace{-3pt}

\section{Problem Formulation}
%This section details the various assumptions and notations that we need in this paper, and the figures of merit for benchmarking a system.
%We start with presenting the general case before turning to the use of embeddings for privacy preserving group membership verification.
%\subsection{About  general group membership verification}
%We impose a few requirements to enforce the generality of our protocol: For security reasons, the enrolled signatures in the database must be protected, that is, they must not be stored in the clear. The same applies to the signatures acquired at authentication time. For privacy reasons, authentication must simply state whether or not the associated user is a member of the group, but it must be impossible to infer which user it is.

% The group membership protocol we present in this paper uses signatures for authenticating users. 
%The exact nature of signatures can vary from one application to the other, and we make quite weak assumptions about them. We simply assume that they are quite complex; they can for example encode information in relation to fingerprints, to the patterns of palm veins, to the faces of individuals, to scans of iris or retinas, to the capture of physical or behavioral traits, or to the specific speckle patterns corresponding to laser-illuminated PUFs.  % Enrollment consists in securely registering (via embedding and aggregation) one signature per user. 
%Verification consists in acquiring a new signature by the client before initiating a comparison process. %and then comparing that newly acquired signature to the ones registered in the database.  
%There are two assumptions, however, that are fundamental to our work:
%the acquired signature at verification time always slightly differs from the one acquired at enrollment time.
%Lighthing conditions, blood pressure, aging, worn-outs, transient physical conditions are possible factors that might cause variations at acquisition time.
%The verification protocol must therefore be able to absorb such variations.
%
%In terms of signal processing, this means that this new signature %querying the database 
%is a noisy version of the one used when that user was enrolled.
%The second assumption we are making is that the signatures corresponding to two different users are always sufficiently dissimilar, and that it is very unlikely that a noisy version of the signature corresponding to one user gets similar enough to the enrolled signature of any other user. These two assumptions are quite general and indeed increase the applicability of our protocol to many real-world situations. 

%A few notations help describing the behavior of a general group membership verification.
Signatures are vectors in $\real^{\dim}$. The dataset is partitioned into $M$ groups. If $m_g$ users/items belong to the $g$-th group, then the protocol considers, $\group_g=\{\x_{1,g}$, \ldots, $\x_{m_{g},g}\}\subset \real^{\dim}$. The signature $\y\in\real^{\dim}$ is a query vector.  Group membership verification considers two hypotheses linked to the continuous nature of the signatures:

$\hyp_{1}$: The query is related to one of the dataset vectors.
For instance, it is a noisy version of vector $j$, $\y=\x_{j}+\n$, with $\n$ to be a noise vector.

$\hyp_{0}$: The query is not related to any vector in the dataset.

%\begin{enumerate}[itemsep=-1mm]
%\item[$\hyp_{1}$:] The query is related to one of the $N$ vectors.
%For instance, it is a noisy version of vector $j$, $\y=\x_{j}+\n$, with $\n$ to be a noise vector. 
%\item[$\hyp_{0}$:] The query is not related to any vector in the group.
%\end{enumerate}

%Section~\ref{sec:OneGroup} studies the aggregation of $N$ signatures into one single representation.
%deals with applications where the $N$ vectors are sketched into is not big so that all vectors can be packed into one group. 
%A group of $N$ vectors is denoted by $\group:=\{\x_{1},\ldots, \x_{N}\}$.
\vspace{4pt}
At the enrollment phase, a group representation learning technique $\func{s}$ computes $M$ representations $\rep_g:= \func{s}(\group_g)$, where $\rep_g$ corresponds to $g$-th group. Variable $\ell$ denotes the size in bits of this representation. %to store this data structure.

At the verification phase, the query $\y$ is hashed by a function $\func{h}$ of size $\ell$ in bits.  This function might be probabilistic to ensure privacy.  The group membership test decides which hypothesis is deemed true by comparing $\func{h}(\y)$ and each ~$\rep_g$.  This is done by first computing a score function $\func{c}$ and thresholding its results: $t:=[\exists g \in [M]$ $\func{c}(\func{h}(\y),\rep_g)>\tau]$.
\vspace{-4pt}







%%% Local Variables:
%%% mode: latex
%%% TeX-master: "GroupMembershipVerification"
%%% End:


==> RelatedWorks.tex <==
% !TEX root = GroupMembershipVerification.tex

\vspace{-3pt}

\section{Related Works}
\label{sec:RelatedWorks}
The combination of group membership verification, continuous vectors, security, and privacy is quite unique.
It is however related to some other fields as found in literature.




% \subsection{Cryptography}
% A group membership verification system can be built on cryptographic primitives.
% That paradigm exhibits several desirable properties. Encryption enforces the security of the data structure stored at the server side.
% %Stealing it is useless: no signature can be decyphered.%; no user can be identified from any encrypted signature.
% Homomorphic encryption allows to compare signatures in the encrypted domain, hence preserving privacy requirements.
% This solution, however, is extremely costly, both in terms of memory footprint (space) and CPU consumption (time).


\vspace{-2pt}

%\subsection{Signal processing in the encrypted domain}
\subsection{Cryptography}
There exist cryptographic protocols setting a key management system to provide the members of a group anonymous authentication~\cite{Schechter:1999qy}.
There is no enrollment of biometric or PUF signatures since membership is equivalent to holding one of the valid keys.
As for biometry or PUF applications, our scenario is different than authentication, identification and secret binding.
These applications secure the signatures at the server and/or the client sides, but ultimately the identity of the user/object is revealed.

Signal processing in the encrypted domain can provide a solution to group membership verification.
Each signature is quantized and protected with homomorphic encryption at the enrollment stage.
The query is protected in the same manner at the verification stage.
This allows to compute distances between the query and the signatures in the encrypted domain~\cite{Troncoso-Pastoriza:2013hi}.
There exist protocols for comparing encrypted results to a threshold~\cite{Erkin:2009cz,Sadeghi:2010bl}.
These encrypted comparisons are sent back to the clients which decrypt to see whether there is at least one positive.      
The security and privacy are as high as the security of the cryptographic primitives.
Cryptography, however, is extremely costly, both in terms of memory footprint (space) and CPU consumption (time).
% Yet, fully-homomorphic encryption is space and time demanding.

\vspace{-2pt}

\subsection{Sketching techniques}
Group membership is linked to the well-known Bloom filter that is used to test whether an element is a member of a set.  A Bloom filter hashes and blends elements into one array of bits.  A Bloom filter can not cause any false negative but makes false positives with a small and tunable probability (reduced at the cost of a larger array of bits). When used in the context of privacy, it was demonstrated that a server using Bloom filters cannot infer any information on one specific entry~\cite{Bianchi:2012sy}.

However, a Bloom filter can not be used as is in our application,  but it needs two adaptations.  First, a Bloom Filter deals with discrete objects whereas we consider continuous high dimensional vectors, the signatures.
We first need to design a quantizer hashing the continuous signatures into discrete objects.
That quantizer must absorb the noise, \ie\ the difference between the enrolled and the fresh signature.
Second, at verification time, the hash of the query cannot be sent in the clear for privacy reasons~\cite{Boneh:2007om}.
Beck and Kerschbaum protect the query with partially homomorphic encryption since there is no need to protect the filter at the server side~\cite{Beck:2013df}. This approach serves as a baseline in our experiments (see Appendix~\ref{sec:BloomFilter}). 



% One has to design a quantizer which casts the continuous signatures into discrete embeddings.
% This has to be robust to noise: the embedding of the query must be identical to the one of the original signature.

% The Bloom filter hashes and blends the enrolled signatures into one data structure s.t. a curious server cannot infer the embedding of one specific entry~\cite{Bianchi:2012sy}.
% Second, at the verification stage, the hash of the query cannot be sent in the clear for security and privacy reasons~\cite{Boneh:2007om}.
% Paper~\cite{Beck:2013df} proposes the protection of the query with partially homomorphic encryption since there is no need to protect the data structure at the server side. This approach will serve as a baseline in our experimental work (see Appendix~\ref{sec:BloomFilter}).
  
  
   \vspace{-2pt}
%\subsection{Signal processing}
\subsection{Aggregating, Embedding}

%The concept of grouping 
Aggregating signals into one representation is a very common mechanism in computer vision. % under the name of aggregation.
Approaches like BoW (Bag of Words)~\cite{Sivic:2003qp}, VLAD~\cite{jegou:inria-00633013}, Fisher vectors~\cite{Perronnin:2007qm}, aggregate some local descriptors extracted from one image into one global description.  However, these approaches are designed to facilitate the identification of similar elements in images and have no security or privacy capabilities. Another recent aggregation method better fits with the security and privacy requirements that we need. In~\cite{iscen:hal-01481220}, Iscen \etal use the \emph{group testing} paradigm to design a strategy for packing a random set of image descriptors into a unique high-dimensional vector. One salient property of that strategy is that the similarity between images can be determined by solely comparing these (few) aggregated vectors to the description of the query, without the need of the original (and numerous) raw image descriptors. Paper~\cite{iscen:hal-01481220} is therefore an excellent basis for the aggregation block that we have mentioned above: the similarities between the original non-aggregated signatures and a query signature is preserved through the aggregation to some extend.
Moreover, it is hard to infer anything about one specific signature from observing the aggregated one.


% A recent paper proposes more compact representations under the name of ``memory vector''~\cite{iscen:hal-01481220}. The representation of a group has indeed the same dimension than the signatures. Packing randomly chosen signatures  provides self-protection: the representation can be seen as one particular signature corrupted by a lot of noise due to the other signatures of the group. 

As for the embedding, our scenario is similar to a privacy-preserving identification mechanism based on sparsifying transform~\cite{Razeghi2017wifs, Razeghi2018icassp}.
%Its consists of a trained/random linear mapper followed by an element-wise nonlinearity. 
It obtains an information-preserving sparse ternary embedding, while ensuring privacy of the data users and security of the signatures. 
%The idea is to project the signature $\mathbf{x} \in \mathbb{R}^{d}$ to the range space of a transform matrix $\mathbf{W} \in \mathbb{R}^{\ell \times d}$, then apply a hard-thresholding operator as to obtain a sparse approximation by keeping the $S_x$ largest magnitudes and setting the remaining low magnitude components to zero. The transform matrix $\mathbf{W}$ is under-complete ($\ell < d$), a square ($\ell = d$), or an over-complete ($\ell > d$) transform, which may reduce, keep, or extend the dimensions, respectively.
%By imposing extra constraint on the alphabet of the embedding as $\{-1, 0, +1 \}$, the hash function $\func{h}_{e}$ can be defined as a projection $\W\x$ followed by a ternarizing sparsifying function $\func{T}_{S_{e}}$, that is:
%\begin{eqnarray}
%\label{eq:EmbedEncoding}
%\func{h}_{e}: \real^{\dim}&\to& \{-1,0, +1\}^{\ell}\\
%\x &\mapsto& \func{h}_{e}(\x) = \func{T}_{S_{e}}(\W\x)\nonumber
%\end{eqnarray}
%The ...
%Moreover, the authors demonstrated that the security of their scheme does not rely on the secrecy of transform. 

This paper pertains to this signal processing approach.
The combination of embedding~\cite{Razeghi2017wifs, Razeghi2018icassp} and aggregation~\cite{iscen:hal-01481220} serves as a baseline. Yet, our paper revisits this approach with machine learning jointly optimizing the embedding and aggregation stages. 

%\textcolor{red}{A citation of Ahmet previous work on identification on group testing.}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "GroupMembershipVerification"
%%% End:


==> introduction.tex <==
% !TEX root = GroupMembershipVerification.tex

\vspace{-4pt}

\section{Introduction}
\label{sec:Introduction}


The verification that an item / device / individual is a member of a group is a natural task which forms the basis of many applications granting or refusing access to buildings or sensitive services.
Group membership verification is \emph{not} about identifying first and then verifying that the item / device / individual is indeed a member of that group. Rather, being granted with a privileged access requires that the members of the group could be distinguished from non-members, but it does not require to distinguish members from one another. Furthermore, privacy concerns suggest that the verification should be carried-out anonymously.

Without any loss of generality, group membership verification protocols need first to
acquire \emph{signatures} of items (passive PUF), devices (active PUF),  or individuals (biometric trait) and to enroll them  into a data structure stored in a server.
Then, at verification time,  that data structure is queried by a client with a new signature and the access is granted or refused.
Security assesses that the data structure is adequately protected so that a honest but curious server cannot reconstruct the signatures.
Privacy requires that verification should proceed without disclosing the identity.
%and such that it is impossible to infer which user it is from the examination of its signature. 

\vspace{-2pt}

% \subsection{Nature of the signatures}
\subsection{Properties of the signatures}

% The group membership protocol we present in this paper uses signatures for authenticating users. 
The nature of signatures can vary from one application to the other.
%, and we make quite weak assumptions about them.
%We simply assume that they are quite complex: they
For example, the signatures encode information related to fingerprints, iris, or faces of individuals, 
%to scans of iris or retinas, to the capture of physical or behavioral traits,
or to speckle patterns captured from laser-illuminated PUFs.  % Enrollment consists in securely registering (via embedding and aggregation) one signature per user. 
%Verification consists in acquiring a new signature by the client before initiating a comparison process. %and then comparing that newly acquired signature to the ones registered in the database.
  
% There are two fundamental difficulties about the s


It is worth highlighting two fundamental properties of the signatures. %we consider in this paper. 
The signature used at verification time is a noisy version of the one acquired at enrollment time.
Lighting conditions, blood pressure, aging, worn-outs, transient physical conditions are possible factors that might cause variations at acquisition time. The verification protocol must be able to absorb such variations and cope with the continuous nature of the signatures. The signatures, however, must be such that it is very unlikely that a noisy version of the signature corresponding to one user gets similar enough to the enrolled signature of any other user. The first property is therefore in relation with the continous and distinguishable nature of the signatures.
%In terms of signal processing, this means that this new signature %querying the database 
%is a noisy version of the one used when that user was enrolled.
The second property is in relation with the statistical independence  of the signatures that are enrolled.
%Signatures ``look like'' random, making their forgery by analysing existing enrolled signatures impossible. 

%Whereas the associated users may share some high-level semantic reason for being members of a group (\eg working in the same building), n

% hard point is that the signatures of a group are statistically independent.
% Although they belong to a group for some semantic reason (\eg signatures of employees working in the same building), they do not reflect this information. These signatures are given by Nature, we have no choice when enrolling them into the data structure.

% and that it is very unlikely that a noisy version of the signature corresponding to one user gets similar enough to the enrolled signature of any other user. These two assumptions are quite general and indeed increase the applicability of our protocol to many real-world situations. 

% \subsection{Security and Privacy}
\subsection{Overview of the contribution}

\vspace{-2pt}

%Our scenario assumes that the client is trusted when acquiring a new signature and querying whereas the server is honest but curious. It tries to reconstruct enrolled signatures from the data structure or the querying signature from the message sent by the client. 


Our scenario considers a server which runs the group membership verification protocol. The server receives queries from clients. A client acquires a new signature
%corresponding to the user whishing to get priviledged access
and then queries the server. Clients are trusted. The server is honest but curious: It may try to reconstruct the enrolled signatures or spy on the queries. % received by the clients.
The protocol
%we present in this paper
intends to prevent the server from inferring any (private) information from the system while correctly determining whether or not a user is a member of the designated group. 
This protocol
%that we detail in the remaining sections of this paper
consists of two main procedures:
%that, all together, succeed in providing a privacy preserving group membership verification system.
%These building blocks can be combined in any order, and the six resulting configurations exhibit different strengths in their ability to enforce the security of the enrollments and preserve the privacy of the information managed at the server and sent by the clients. 
\begin{itemize}
	\item \emph{Embedding}: It hashes signatures into discrete \emph{embeddings}. Quantization is a lossy process limiting the ability of the server to reconstruct signatures. %from the embeddings.
	\item \emph{Aggregation}: It aggregates multiple signatures into a unique representation. The server can  not infer any specific signature from this aggregated information.
\end{itemize}
At verification time, the information received by a client is used against such group representations. The aggregation process must preserve sufficient information %, such that the server remain able
to assert whether or not the queried signature is a member of the group.
This paper proposes to jointly learn both processes under two configurations that differ on the ordering:
%by proposing two schemes. The basic idea of proposed schemes is based on ordering of the above processes, where we can have two configurations:
\begin{itemize}
	\item \emph{Aggregation of Embedding}: The signatures of the group are hashed before being aggregated into a unique representation.
	\item \emph{Embedding of Aggregation}: Signatures are aggregated and then the result of this aggregation is hashed.
\end{itemize} 
The weaknesses and strengths of these two configurations are explored in the following sections.


% This paper proposes a very different approach based on signal processing techniques.
% It trades security and privacy for a lower cost in space and time.
% % resulting in the design of a privacy preserving group membership verification protocol. It does
% %not relying on any form on encryption. It rather fully uses signal processing techniques.
% %To enforce the security of the signatures and to forbid any possible reconstruction,

% The security of this approach relies on three mechanisms.
% First, the continuous signatures are hashed into discrete \emph{embeddings}.
% This amounts to a quantization which prevents reconstruction of the signatures to some extend.
% At the enrollment, the \emph{aggregation} of signatures into a data structure plays a self-protection.
% It is not possible to isolate one particular signature.
% Since this approach is robust to noise, \emph{insertion of noise} by the client strengthens the privacy of the querying signature. 
 

%Verification then boils down to evaluating the similarities between the embedding of the query signature and the representatives. If a high enough similarity is observed, then it is proved that this signature has been enrolled, otherwise it is unknown.
%Considering representatives allows to assess whether or not a user is a member of a group and forbids its exact identification.

%{\color{red} Role of the client.}
 



% relies on separating all the enrolled signatures into disjoint \emph{signature-groups} before aggregating the multiple signatures of one  group into a unique \emph{super-signature}, also called a \emph{memory vector}. Verification then boils down to evaluating the similarities between the query signature and the \emph{memory vectors}. If a high enough similarity is observed, then it is proved that the query signature has indeed been enrolled. Otherwise the user is unkown. 

%In contrast to encryption, signal processing cause negligible overhead, space and CPU wise. **another cool property?** Experiments show that...

%The rest of this paper is...


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "GroupMembershipVerification"
%%% End:

